Fine-grained Private Knowledge Distillation

Knowledge distillation has emerged as a scalable and effective way for privacy-preserving machine learning. One remaining drawback is that it consumes privacy in a model-level (i.e., client-level) manner, every distillation query incurs privacy loss of one client's all records. In order to attain fine-grained privacy accountant and improve utility, this work proposes a model-free reverse $k$-NN labeling method towards record-level private knowledge distillation, where each record is employed for labeling at most $k$ queries. Theoretically, we provide bounds of labeling error rate under the centralized/local/shuffle model of differential privacy (w.r.t. the number of records per query, privacy budgets). Experimentally, we demonstrate that it achieves new state-of-the-art accuracy with one order of magnitude lower of privacy loss. Specifically, on the CIFAR-$10$ dataset, it reaches $82.1\%$ test accuracy with centralized privacy budget $1.0$; on the MNIST/SVHN dataset, it reaches $99.1\%$/$95.6\%$ accuracy respectively with budget $0.1$. It is the first time deep learning with differential privacy achieve comparable accuracy with reasonable data privacy protection (i.e., $\exp(\epsilon)\leq 1.5$). Our code is available at https://github.com/liyuntong9/rknn.

==> abandon.tex <==

\subsection{An Improved Oracle for Low Privacy}
When the privacy level is relatively low (e.g., when $\epsilon>1$ with shuffling privacy amplification in the next section), due to the information loss of sampling in Equation (\ref{eq:collision}), the Collision mechanism for set-valued summation is sub-optimal. Specifically even when $\epsilon=+\infty$, the mean squared error of $A^i$ is $k^2 r^2-k r$, which is greater than $0$ as expected. In this part, based on a flexible utility function design in the framework of exponential mechanism \cite{mcsherry2007mechanism,wang2018privset},  we propose the General Subset Exponential (GSE) mechanism to achieve improved utility in the low privacy regime.

As Definition \ref{def:gse} implied, given as input a size-$m$ subset $V$ of the domain $\mathcal{G}$, the GSE mechanism outputs a size-$l$ subset $Z\subseteq \mathcal{G}$. When the cardinality of $V \cap Z$ is at least $\alpha_{min} \in \mathbb{N}^+$, the output probability of $Z$ is proportional to $e^\epsilon$. Otherwise, the the output probability of $Z$ is proportional to $1$.   

\begin{definition}[$(d,c,\epsilon,l,\alpha_{min})$-GSE Mechanism]\label{def:gse}
Take a vector $V$ having $c$ non-zero entries as input ($V \subseteq \mathcal{G}$), the GSE mechanism randomly outputs a subset $Z \subseteq \mathcal{G}$ according to following probability design:
\begin{equation}\label{eq:gse}
    \mathbb{P}[Z | V]= \left\{
    \begin{array}{@{}lr@{}}
        \frac{e^\epsilon}{\Omega},\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \text{if } |Z|=l\ and\ |Z\cap V|\geq \alpha_{min};\\
        \frac{1}{\Omega},\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \text{if } |Z|=l\ and\ |Z\cap V|< \alpha_{min};\\
        0.\ \ \ \  \ \ \ \  \ \ \ \  \ \ \ \  \ \ \ \  \ \ \ \  \ \ \ \  \ \ \ \  \ \ \ \  \ \ \ \  \ \ \ \  \ \ \ \ \ \ \ otherwise.\\
    \end{array}
    \right.
\end{equation}
The normalization factor is $\Omega=e^\epsilon\sum_{i=\alpah_min}^{c}{c\choose i}{d-c \choose l-i}+\sum_{i=0}^{\alpah_min}{c\choose i}{d-c \choose l-i}$. For any $v \in \mathcal{G}$, an unbiased estimator of the indicator $\llbracket v\in V\rrbracket$ is $\tilde{\llbracket v \in V\rrbracket}=\frac{\llbracket v\in Z\rrbracket- p_{f}}{p_{t}-p_{false}}$, where $p_{t}=\frac{e^\epsilon\sum_{i=\alpah_min}^{c}{c-1\choose i-1}{d-c \choose l-i}+\sum_{i=0}^{\alpah_min}{c-1\choose i-1}{d-c \choose l-i}}{\Omega}$ and $p_{f}=\frac{e^\epsilon\sum_{i=\alpah_min}^{c}{c\choose i}{d-c-1 \choose l-i-1}+\sum_{i=0}^{\alpah_min}{c\choose i}{d-c-1 \choose l-i-1}}{\Omega}$.
\end{definition}

Properly setting the subset size parameter $l$ and threshold $\alpha_{min}$ in the GSE mechanism could optimizes the estimation error for set-valued summation. Specifically, when $\alpha_{min}$ is fixed at $1$, the GSE mechanism is identical to \cite{wang2018privset}, which dominates the Collision mechanism when $\epsilon=O(1)$. Therefore, the $(s\cdot |\mathcal{Y}|,k\cdot r,\epsilon,2k\cdot r-1+k\cdot r\cdot e^\epsilon,1)$-GSE mechanism is also an $(O(\sqrt{\frac{m k r \log(|\mathcal{Y}|/\beta)}{\epsilon^2}}), \beta)$-accurate algorithm for the bucketized sparse vector summation problem when $\epsilon=O(1)$. In Figure \ref{fig:mse}, we demonstrate the theoretical mean squared errors of set-valued summation when domain size is $d=16$ and maximum cardinality is $c=4$. It is observed that the GSE mechanism significantly outperforms the Collision mechanism when the privacy budget is relatively large.




Naively, we could also adopt the Laplace mechanism for preserving local $\epsilon$-DP, and add $Laplace(\frac{2\cdot k \cdot r}{\epsilon})$ to every value in $A^i$. We show the Laplace mechanism is $(\max\{\sqrt{\frac{8\log(|\mathcal{Y}|/\beta) k^2 r^2 m^2}{\epsilon^2}}, \frac{4\log(|\mathcal{Y}|/\beta) k r}{\epsilon}\},\beta)$-accurate in Proposition \ref{pro:locallaplace}, which is derived from the additive property and the tail bounds of sub-exponential variables.

\begin{proposition}\label{pro:locallaplace}
The Laplace mechanism with local $\epsilon$-DP is an $(\max\{\sqrt{\frac{8\log(|\mathcal{Y}|/\beta) k^2 r^2 m^2}{\epsilon^2}}, \frac{4\log(|\mathcal{Y}|/\beta) k r}{\epsilon}\}, \beta)$-accurate algorithm for bucketized sparse vector summation problem. The running time for one datum is $poly(|T|, r)$.
\end{proposition}
\begin{proof}
Recall that $v\sim Laplace(0,\frac{\epsilon}{k\cdot r})$ is $((\frac{2k\cdot r}{\epsilon})^2,\frac{2k\cdot r}{\epsilon})$-sub-exponential. That is:
$$\mathbb{E}[e^{\lambda v}]\leq e^{(\frac{2k\cdot r}{\epsilon})^2\frac{\lambda^2}{2}},\ \ \ \ \ \  \forall\  |\lambda|\leq \frac{\epsilon}{2k\cdot r}.$$ According to the additive proper of independent sub-exponential variables, we have $u \sim \sum_{i=1}^{m} Laplace(0,\frac{\epsilon}{k\cdot r})$ is $(m(\frac{2k\cdot r}{\epsilon})^2, \frac{2k\cdot r}{\epsilon})$-sub-exponential.
Then, based on the tail bounding of sub-exponential variables, we have $\mathbb{P}[|u|\geq \eta\cdot m]\leq \exp(-\frac{m}{2}\min\{\frac{\eta^2{\epsilon}^2}{m({2k\cdot r})^2},\frac{\eta \epsilon}{2k\cdot r}\})$. Finally, for a vector of variables,  $U=\{u_1,u_2,...,u_{|\mathcal{Y}|}\}$ that $u_j$ is summation of $m$ independent variables as $\sum_{i=1}^{m} Laplace(0,\frac{\epsilon}{k\cdot r})$, we have $\mathbb{P}[\max_{j=1}^{|\mathcal{Y}|} |u_j|\geq \eta\cdot m]\leq |\mathcal{Y}|\cdot\exp(-\frac{m}{2}\min\{\frac{\eta^2{\epsilon}^2}{m({2 k r})^2},\frac{\eta \epsilon}{2k r}\})$. Hence, with probability $1-\beta$, we have $\max_{j=1}^{|\mathcal{Y}|} |u_j| \leq \max\{\sqrt{\frac{8\log(|\mathcal{Y}|/\beta) k^2 r^2 m^2}{\epsilon^2}}, \frac{4\log(|\mathcal{Y}|/\beta) k r}{\epsilon}\}$.
\end{proof}

Similarly, when adopt the classical randomized response mechanism \cite{warner1965randomized,duchi2013local} for preserving local $\epsilon$-DP, and randomly flip every binary value in $A^i$ with probability $\frac{1}{e^{\epsilon/(2k r)}+1}$, it is $(O(\sqrt{\frac{m k^2 r^2\log(|\mathcal{Y}|/\beta)}{ \epsilon^2}}),\beta)$-accurate (see Proposition \ref{pro:rr}).



